Intent Identification and Entity Extraction for Healthcare Queries in Indic Languages

Scarcity of data and technological limitations for resource-poor languages in developing countries like India poses a threat to the development of sophisticated NLU systems for healthcare. To assess the current status of various state-of-the-art language models in healthcare, this paper studies the problem by initially proposing two different Healthcare datasets, Indian Healthcare Query Intent-WebMD and 1mg (IHQID-WebMD and IHQID-1mg) and one real world Indian hospital query data in English and multiple Indic languages (Hindi, Bengali, Tamil, Telugu, Marathi and Gujarati) which are annotated with the query intents as well as entities. Our aim is to detect query intents and extract corresponding entities. We perform extensive experiments on a set of models in various realistic settings and explore two scenarios based on the access to English data only (less costly) and access to target language data (more expensive). We analyze context specific practical relevancy through empirical analysis. The results, expressed in terms of overall F1 score show that our approach is practically useful to identify intents and entities.

==> tables/few_shot_merged_table.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{| l | l | cccc | cccc || cccc | cccc |}\toprule
\multirow{3}{*}{Lang} &\multirow{3}{*}{Models} &\multicolumn{8}{c||}{Intent} &\multicolumn{8}{c|}{Entity} \\
\cmidrule(r){3-10}
\cmidrule(r){11-18}
& &\multicolumn{4}{c|}{WebMD} &\multicolumn{4}{c||}{1mg} &\multicolumn{4}{c|}{WebMD} &\multicolumn{4}{c|}{1mg} \\
% \cmidrule(r){3-6}
% \cmidrule(r){7-10}
% \cmidrule(r){11-14}
% \cmidrule(r){15-18}
\cmidrule(r){3-10}
\cmidrule(r){11-18}
& &20\% &40\% &60\% &80\% &20\% &40\% &60\% &80\% &20\% &40\% &60\% &80\% &20\% &40\% &60\% &80\% \\\midrule
\multirow{2}{*}{Hi} &mBERT &59.03 &60.21 &57.75 &59.22 &62.11 &58.38 &46.83 &68.78 &6.24 &22.11 &19.69 &15.94 &33.20 &43.37 &47.82 &51.07 \\ 
&XLM-R &70.58 &64.25 &67.06 &70.24 &42.56 &41.29 &49.17 &41.02 &21.95 &30.24 &30.19 &37.81 &68.52 &55.87 &66.52 &71.78 \\\bottomrule
\multirow{2}{*}{Bn} &mBERT &49.02 &59.87 &62.17 &62.83 &51.78 &50.68 &41.18 &66.66 &17.54 &16.33 &16.67 &28.77 &48.05 &51.82 &63.62 &57.85 \\
&XLM-R &62.61 &14.31 &64.04 &14.31 &54.61 &40.61 &41.41 &46.28 &28.83 &38.89 &35.92 &49.44 &63.68 &66.91 &69.14 &71.32 \\\bottomrule
\multirow{2}{*}{Ta} &mBERT &52.84 &57.14 &54.20 &57.73 &61.83 &57.35 &56.37 &54.28 &0.00 &0.00 &0.00 &0.00 &42.42 &43.27 &48.31 &46.21 \\
&XLM-R &64.86 &59.70 &63.38 &67.41 &55.70 &45.34 &41.76 &40.48 &31.97 &27.64 &24.25 &19.89 &67.03 &66.56 &69.99 &68.40 \\\bottomrule
\multirow{2}{*}{Te} &mBERT &57.16 &65.92 &64.87 &64.06 &54.93 &53.03 &42.35 &51.19 &6.00 &0.00 &0.00 &0.00 &16.78 &16.78 &16.78 &20.49 \\
&XLM-R &52.84 &57.14 &54.20 &57.73 &49.49 &47.65 &57.13 &48.81 &46.87 &29.46 &30.72 &32.82 &64.26 &66.83 &68.52 &63.35 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{(Setup 6) Macro-F1 scores for Mixed Language Train Setting English and Indic with various percentage split. XLM-R indicates XLM-RoBERTa, WMD indicates WebMD}
\vspace{-3mm}
\end{table*}




% \begin{table*}[t]
% \large
% \footnotesize
% \centering

% \begin{tabular}{ l l cccc cccc}
% \toprule
% & & \multicolumn{4}{c}{WebMD} & \multicolumn{4}{c}{1mg} \\
% \cmidrule(r){3-6}
% \cmidrule(r){7-10}
% %\cmidrule(r){14-17}
% Lang & Models & 20\% & 40\% & 60\% & 80\% & 20\% & 40\% & 60\% & 80\%\\
% \midrule
% %En & mBERT &  &  &  &  & &  &  & &\\
%   % & XLM-R &  &  &  &  & &  &  & &\\
% %\midrule
% Hi & mBERT &59.03  &60.21  &57.75  &59.22  & 62.11  & 58.38  & 46.83 & 68.78\\
%     & XLM-R &70.58  &64.25  &67.06  &70.24   & 42.56  & 41.29  & 49.17 & 41.02\\
% \midrule
% Bn & mBERT  &49.02  &59.87  &62.17  &62.83 & 51.78  & 50.68 & 41.18 &66.66\\
%     & XLM-R &62.61  &14.31  &64.04  &14.31  & 54.61  & 40.61  & 41.41 & 46.28\\
% \midrule
% Ta & mBERT  &52.84  &57.14  &54.20  &57.73 &  61.83  & 57.35 & 56.37 & 54.28\\
%     & XLM-R &64.86  &59.70  &63.38  &67.41   &55.70  & 45.34  & 41.76 & 40.48\\
% \midrule
% Te & mBERT  &57.16  &65.92  &64.87  &64.06  & 54.93  & 53.03 & 42.35 & 51.19\\
%     & XLM-R &52.84  &57.14  &54.20  &57.73   & 49.49  & 47.65  & 57.13 & 48.81\\
% \bottomrule
% \end{tabular}
% \caption{Results of Few-Shot Experiments using m-BERT and XLM-R on Intent Classification varying the percentage of the queries of the target language in the Training Data. For instance, 20\% indicates that the training set comprises of 20\% queries in the Target Language and 80\% in English.}
% % manually written Kikuyu queries to ``\emph{Pivot}" language.}}
% \label{tab:results}
% \end{table*}




% \begin{table*}[t]
% \footnotesize
% \centering
% \begin{tabular}{ l l cccc cccc}
% \toprule
% & & \multicolumn{4}{c}{WebMD} & \multicolumn{4}{c}{1mg} \\
% \cmidrule(r){3-6}
% \cmidrule(r){7-10}
% %\cmidrule(r){14-17}
% Lang & Models & 20\% & 40\% & 60\% & 80\% &  20\% & 40\% & 60\% & 80\% \\
% \midrule
% %En & mBERT &  &  &  &  & &  &  & &\\
%   %& XLM-R &  &  &  &  & &  &  & &\\
% %\midrule
% Hi & mBERT & 6.24 & 22.11 & 19.69 & 15.94   & 33.20 & 43.37 & 47.82 & 51.07  \\
%     & XLM-R & 21.95 & 30.24 & 30.19 & 37.81  & 68.52 & 55.87 & 66.52 & 71.78  \\
%     % & iBERT & 0.00 & 13.79 & 8.71 & 8.79 & & 0.00 & 4.52 & 12.59 & 4.52 & \\
% \midrule
% Bn & mBERT  & 17.54 & 16.33 & 16.67 & 28.77 &    48.05 & 51.82 & 63.62 & 57.85 \\
%     & XLM-R & 28.83 & 38.89 & 35.92 & 49.44 &  63.68 & 66.91 & 69.14 & 71.32 \\
%     % &  iBERT &  &  &  &  & & 0.00 & 36.57 & 31.09 & 29.37 & \\
% \midrule
% Ta & mBERT  & 0.00 & 0.00 & 0.00 & 0.00 &   42.42 & 43.27 & 48.31 & 46.21   \\
%     & XLM-R & 31.97 & 27.64 & 24.25 & 19.89 &  67.03 & 66.56 & 69.99 & 68.40  \\
%     % &  iBERT & 0.00 & 3.21 & 0.00 & 0.00 & & 0.00 & 39.89 & 41.65 & 41.65 & \\
% \midrule
% Te & mBERT  & 6.00 & 0.00 & 0.00 & 0.00 &   16.78  & 16.78 & 16.78 & 20.49  \\
%     & XLM-R & 46.87 & 29.46 & 30.72 & 32.82 &  64.26 & 66.83 & 68.52 & 63.35  \\
%     % &  iBERT & 3.22 & 0.00 & 0.00 & 0.00 & & 0.00 & 35.89 & 39.89 & 46.98 & \\
% \bottomrule
% \end{tabular}
% \caption{Results of Few-Shot Experiments using m-BERT and XLM-R on Entity Recognition varying the percentage of the queries of the target language in the Training Data. For instance, 20\% indicates that the training set comprises of 20\% queries in the Target Language and 80\% in English.}
% % manually written Kikuyu queries to ``\emph{Pivot}" language.}}
% \label{tab:results}
% \end{table*}





==> tables/new_setup5_table.tex <==
\iffalse{}
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l |cccc| cccc|}\toprule
\multirow{3}{*}{Lang} &\multicolumn{4}{c|}{Intent} &\multicolumn{4}{c|}{Entity} \\
\cmidrule(r){2-9}
% \cmidrule{2-9}
% \cmidrule(r){6-9}
&\multicolumn{2}{c}{mBERT} &\multicolumn{2}{c|}{XLM-R} &\multicolumn{2}{c}{mBERT} &\multicolumn{2}{c|}{XLM-R} \\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
&WMD &1mg &WMD &1mg &WMD &1mg &WMD &1mg \\\midrule
En &70.02 &63.73 &74.44 &53.89 &42.47 & 56.83 &52.37 &59.21 \\
Hi &63.12 &61.54 &62.36 &41.88 &21.34 &49.63 &35.87 &71.64 \\
Bn &63.95 &54.65 &14.31 &50.21 &24.17 &63.84 &46.21 &70.48 \\
Ta &62.97 &63.98 &65.03 &40.81 &0.00 &52.86 &39.83 &68.94 \\
Te &56.11 &58.45 &58.22 &42.58 &0.00 &20.49 &28.53 &46.37 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{(Setup 5) Train and Test on Indic Languages}
\vspace{-2mm}
\end{table}
\fi
